Neural Point Light Fields

We introduce Neural Point Light Fields that represent scenes implicitly with a light field living on a sparse point cloud. Combining differentiable volume rendering with learned implicit density representations has made it possible to synthesize photo-realistic images for novel views of small scenes. As neural volumetric rendering methods require dense sampling of the underlying functional scene representation, at hundreds of samples along a ray cast through the volume, they are fundamentally limited to small scenes with the same objects projected to hundreds of training views. Promoting sparse point clouds to neural implicit light fields allows us to represent large scenes effectively with only a single radiance evaluation per ray. These point light fields are a function of the ray direction, and local point feature neighborhood, allowing us to interpolate the light field conditioned training images without dense object coverage and parallax. We assess the proposed method for novel view synthesis on large driving scenarios, where we synthesize realistic unseen views that existing implicit approaches fail to represent. We validate that Neural Point Light Fields make it possible to predict videos along unseen trajectories previously only feasible to generate by explicitly modeling the scene.

==> fabrication.tex <==
\subsection{Lens Fabrication}
%
\begin{itemize}
	\item Fabrication process.
	\item Imperfections.
\end{itemize}

\paragraph{Experimental Setup}
%
\begin{itemize}
	\item Hardware prototype description.
	\item Sensor readout and ISP pre-processing.
\end{itemize}

\subsection{Learned Calibration}
%
\begin{itemize}
	\item Monitor setup.
	\item Learning procedure and comparison against PSF calibration.
\end{itemize}

